Training-Free Zero-Shot Temporal Action Detection with Vision-Language Models

Existing zero-shot temporal action detection (ZSTAD) methods predominantly use fully supervised or unsupervised strategies to recognize unseen activities. However, these training-based methods are prone to domain shifts and require high computational costs, which hinder their practical applicability in real-world scenarios. In this paper, unlike previous works, we propose a training-Free Zero-shot temporal Action Detection (FreeZAD) method, leveraging existing vision-language (ViL) models to directly classify and localize unseen activities within untrimmed videos without any additional fine-tuning or adaptation. We mitigate the need for explicit temporal modeling and reliance on pseudo-label quality by designing the LOGarithmic decay weighted Outer-Inner-Contrastive Score (LogOIC) and frequency-based Actionness Calibration. Furthermore, we introduce a test-time adaptation (TTA) strategy using Prototype-Centric Sampling (PCS) to expand FreeZAD, enabling ViL models to adapt more effectively for ZSTAD. Extensive experiments on the THUMOS14 and ActivityNet-1.3 datasets demonstrate that our training-free method outperforms state-of-the-art unsupervised methods while requiring only 1/13 of the runtime. When equipped with TTA, the enhanced method further narrows the gap with fully supervised methods.

==> algorithms/adazad.tex <==
\small
\caption{\small Adaptation-Based Zero-Shot TAD }
\label{alg:adazad}
%\algcomment{\fontsize{7.2pt}{0em}\selectfont \texttt{alpha\_cumprod(t)}: cumulative product of $\alpha_i$, \ie, $\prod_{i=1}^t \alpha_i$}
\definecolor{codeblue}{rgb}{0.25,0.5,0.5}
\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codekw}{RGB}{207,33,46}
\lstset{
  backgroundcolor=\color{white},
  basicstyle=\fontsize{7.5pt}{7.5pt}\ttfamily\selectfont,
  columns=fullflexible,
  breaklines=true,
  captionpos=b,
  commentstyle=\fontsize{7.5pt}{7.5pt}\color{codegreen},
  morekeywords={avg},
  keywordstyle=\fontsize{7.5pt}{7.5pt}\color{codekw},
  escapechar={|}, 
}
\begin{lstlisting}[language=python]
def AdaZAD(video, text):
  """
  video: [T, H, W, 3]
  text: [C]
  # T: number of frames
  # C: number of action categories
  """
  
  vis_feat = video_embedding(video)
  text_feat = text_embedding(text)
  
  video_vis = avg (vis_feat)
  cls = cos (video_vis, text_feat)
  label = argmax (cls)
  prototype = text_feat[label]

  # Test-time Adaptation
  for i in range (M):
    sim = norm (cos (vis_feat, prototype))
    # Prototype-centric sampling
    sim_p, sim_n, feat_p = PCS (sim, vis_feat)
    video_proj, text_proj 
      = loss (feat_p, prototype) 
      + loss (sim_p, sim_n, sim_binary)
    vis_feat = video_proj (vis_feat)
    proto = text_proj (proto)

  sim = norm (cos (vis_feat, proto))
  segment = filt (sim)

  p = LogOIC (sim, segment)
  s = actionness_calibration (vis_feat, segment)
  confidence = p * s

  return segment, confidence
\end{lstlisting}

\begin{comment}
\begin{algorithm}[ht]
\caption{Adaptation-based Zero-shot TAD}
\label{alg_enhance}
\begin{algorithmic}
\STATE \texttt{def AdaZAD (video, text):}\\
\hspace{1em} \texttt{vis\_feat = video\_encoder(video)}\\
\hspace{1em} \texttt{text\_feat = text\_encoder(text)}\\
\hspace{1em} \\
\hspace{1em} \# \texttt{Video-level classification}\\
\hspace{1em} \texttt{video\_vis = avg (vis\_feat)}\\
\hspace{1em} \texttt{class = cos (video\_vis, text\_feat)}\\
\hspace{1em} \texttt{label = argmax (class)}\\
\hspace{1em} \texttt{proto = text\_feat[label]}\\
\hspace{1em} \\
\hspace{1em} \# \textbf{\texttt{Test-time Adaptation}}\\
\hspace{1em} \texttt{for i in range (T):}\\
\hspace{2em} \texttt{sim = norm (cos (vis\_feat, proto))}\\
\hspace{1em} \\
\hspace{2em} \# \textbf{\texttt{Prototype-centric sampling}}\\
\hspace{2em} \texttt{sim$^{+}$, sim$^{-}$ = pc\_select (sim)}\\
\hspace{2em} \texttt{feat$^{+}$ = pc\_select (sim, vis\_feat)}\\
\hspace{2em} \texttt{video\_proj, text\_proj}\\
\hspace{3em} \texttt{= loss (feat$^{+}$, proto)}\\
\hspace{3em} \texttt{+ loss (sim$^{+}$, sim$^{-}$, sim\_binary)}\\
\hspace{2em} \texttt{vis\_feat = video\_proj (vis\_feat)}\\
\hspace{2em} \texttt{proto = text\_proj (proto)}\\
\hspace{1em} \\
\hspace{1em} \# \texttt{Action localization}\\
\hspace{1em} \texttt{sim = norm (cos (vis\_feat, proto))}\\
\hspace{1em} \texttt{segment = filter ($\alpha$, sim)}\\
\hspace{1em} \\
\hspace{1em} \# \texttt{Confidence generation}\\
\hspace{1em} \# \texttt{Logarithmic decay weighted OIC}\\
\hspace{1em} \texttt{seg\_out = extansion (segment)}\\
\hspace{1em} \texttt{w = LDW (seg\_out, segment)}\\
\hspace{1em} \texttt{s\_in = avg ( sim[segment])}\\
\hspace{1em} \texttt{s\_out = avg ( w $\times$ sim[seg\_out])}\\
\hspace{1em} \texttt{p = s\_in - 0.2 $\times$ s\_out + max(sim)}\\
\hspace{1em} \# \texttt{Actionness calibration}\\
\hspace{1em} \texttt{z = fft (vis\_feat[segment])}\\
\hspace{1em} \texttt{s = sigmoid (avg (z))}\\
\hspace{1em} \texttt{confidence = p $\times$ s}\\
\hspace{1em} \\
\hspace{1em} \texttt{return segment, confidence}
\end{algorithmic}
\end{algorithm}
\end{comment}

==> algorithms/freezad.tex <==
\small
\caption{\small Training-free Zero-shot TAD }
\label{alg:freezad}
%\algcomment{\fontsize{7.2pt}{0em}\selectfont \texttt{alpha\_cumprod(t)}: cumulative product of $\alpha_i$, \ie, $\prod_{i=1}^t \alpha_i$}
\definecolor{codeblue}{rgb}{0.25,0.5,0.5}
\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codekw}{RGB}{207,33,46}
\lstset{
  backgroundcolor=\color{white},
  basicstyle=\fontsize{7.5pt}{7.5pt}\ttfamily\selectfont,
  columns=fullflexible,
  breaklines=true,
  captionpos=b,
  commentstyle=\fontsize{7.5pt}{7.5pt}\color{codegreen},
  morekeywords={avg},
  keywordstyle=\fontsize{7.5pt}{7.5pt}\color{codekw},
  escapechar={|}, 
}
\begin{lstlisting}[language=python]
def FreeZAD(video, text):
  """
  video: [T, H, W, 3]
  text: [C]
  # T: number of frames
  # C: number of action categories
  """
  
  # Feature embedding
  vis_feat = video_embedding(video)
  text_feat = text_embedding(text)
  
  # Video-level classification
  video_vis = avg (vis_feat)
  cls = cos (video_vis, text_feat)
  label = argmax (cls)
  prototype = text_feat[label]

  # Action localization
  sim = norm (cos (vis_feat, prototype))
  segment = filt (sim)

  # Confidence generation
  p = LogOIC (sim, segment)
  s = actionness_calibration (vis_feat, segment)
  confidence = p * s

  return segment, confidence
\end{lstlisting}

\begin{comment}
\begin{algorithm}[ht]
\caption{Training-free Zero-shot TAD}
\label{alg_freezad}
\begin{algorithmic}
\STATE \texttt{def FreeZAD (video, text):}\\
\hspace{1em} \texttt{vis\_feat = video\_encoder(video)}\\
\hspace{1em} \texttt{text\_feat = text\_encoder(text)}\\
\hspace{1em} \\
\hspace{1em} \# \textbf{\texttt{Video-level classification}}\\
\hspace{1em} \texttt{video\_vis = avg (vis\_feat)}\\
\hspace{1em} \texttt{class = cos (video\_vis, text\_feat)}\\
\hspace{1em} \texttt{label = argmax (class)}\\
\hspace{1em} \texttt{proto = text\_feat[label]}\\
\hspace{1em} \\
\hspace{1em} \# \textbf{\texttt{Action localization}}\\
\hspace{1em} \texttt{sim = norm (cos (vis\_feat, proto))}\\
\hspace{1em} \texttt{segment = filter ($\alpha$, sim)}\\
\hspace{1em} \\
\hspace{1em} \# \textbf{\texttt{Confidence generation}}\\
\hspace{1em} \# \texttt{Logarithmic decay weighted OIC}\\
\hspace{1em} \texttt{seg\_out = extansion (segment)}\\
\hspace{1em} \texttt{w = LDW (seg\_out, segment)}\\
\hspace{1em} \texttt{s\_in = avg ( sim[segment])}\\
\hspace{1em} \texttt{s\_out = avg ( w $\times$ sim[seg\_out])}\\
\hspace{1em} \texttt{p = s\_in - 0.2 $\times$ s\_out + max(sim)}\\
\hspace{1em} \# \texttt{Actionness calibration}\\
\hspace{1em} \texttt{z = fft (vis\_feat[segment])}\\
\hspace{1em} \texttt{s = sigmoid (avg (z))}\\
\hspace{1em} \texttt{confidence = p $\times$ s}\\
\hspace{1em} \\
\hspace{1em} \texttt{return segment, confidence}
\end{algorithmic}
\end{algorithm}
\end{comment}
